Monocular Camera Based Fruit Counting and Mapping with Semantic Data Association

We present a cheap, lightweight, and fast fruit counting pipeline that uses a single monocular camera. Our pipeline that relies only on a monocular camera, achieves counting performance comparable to state-of-the-art fruit counting system that utilizes an expensive sensor suite including LiDAR and GPS/INS on a mango dataset. Our monocular camera pipeline begins with a fruit detection component that uses a deep neural network. It then uses semantic structure from motion (SFM) to convert these detections into fruit counts by estimating landmark locations of the fruit in 3D, and using these landmarks to identify double counting scenarios. There are many benefits of developing a low cost and lightweight fruit counting system, including applicability to agriculture in developing countries, where monetary constraints or unstructured environments necessitate cheaper hardware solutions.

==> tex/Acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:acknowledgements}
This work was supported by USDA NIFA grant 2015-67021-23857 under the National Robotics Initiative, Semiconductor Research Corporation (SRC), and the Australian Centre for Field Robotics (ACFR) at The University of Sydney, with thanks to Simpsons Farms. 


==> tex/ProblemFormulation.tex <==

\section{Problem Formulation}
Consider a sequence of $n$ images $\mathbfcal{I} = (\mathcal{I}_{k})_{k=1}^{n}$ of trees containing fruit of the same type. The image sequence $\mathbfcal{I}$ has a state $\mathbf{z} \in \mathbb{N}$ representing the actual filed count of fruits on trees in this image sequence $\mathbfcal{I}$. 


\textbf{Fruit Counting:} Given a set of $m$ image sequences $\{\mathbfcal{I}^{(j)}\}_{j=1}^{m}$, our goal is to find the mapping $f \colon \mathbfcal{I}^{(j)} \rightarrow \mathbf{z}^{(j)} \in \mathbb{N}$ to produce filed count from the image sequence set. The discrepancy between this estimate  $\mathbf{z}^{(j)}$ and the true visual count $\hat{\mathbf{z}}^{(j)}$ is captured through the L1 loss, defining the metric used for the evaluation of our algorithm. 
\begin{equation}
%\sum_{j=1}^{m}|f(\mathbf{\mathcal{I}}^{(j)})-\mathbf{z}^{(j)}|
\sum_{j=1}^{m}|f(\mathbf{\mathcal{I}}^{(j)})-\hat{\mathbf{z}}^{(j)}|
%\vspace*{-0.1in}
\end{equation}

==> tex/ProposedApproach.tex <==


\section{Outline of Proposed Approach}
Our objective is to estimate the field counts of fruits on trees. We limit ourselves to using only a monocular camera, which presents additional challenges over the previous work in ~\cite{stein2016image} since depth information or pose information is not directly available from a LiDAR or GPS/INS sensors. Our previous  monocular camera fruit counting approach first maintains fruit tracks in the 2D image plane across frames. Separately, to reject outlier fruits, a computationally expensive structure from motion (SFM) reconstruction is performed using relatively dense SIFT features~\cite{liu2018robust}. However, in this approach, the counting and data association is still performed in 2D and the 3D points are reconstruction of SIFT features, not fruits. We unify our two previous works by using a monocular camera to estimate the camera pose and fruit landmark locations and perform 3D-2D data association and 3D-landmark-based counting. This method can decrease computation time and increase accuracy. Our algorithm can be broken down into two components: (1) robustly detect fruits in a given image, and (2) associate each detected fruit with a 3D landmark in order to identify double counting scenarios. 

%To maximize the probablity of detecting all fruits on a given tree, our dataset features multiple views taken from both sides of the tree. The role of the 3D landmark association is thus to prevent double-counting of fruits that result from viewing the same fruit from multiple views on the same side of the tree, as well as from opposite sides of the tree. 
%In the first step, we used the Faster R-CNN (FR-CNN), a state-of-the-art object detector, to detect fruits. In the second step, we generate a 3D landmark for every detected fruit. The 3D landmarks are used to get both the data association across frames to avoid double counting from multiple views from one side of trees, and the spatial relationship between the landmarks and tree centroids to avoid double counting from two opposite sides of the same trees.

%Our pipeline consists of two systems: The fruit detection system and the fruit landmark based counting system. The fruit detection system detect fruits in every image using the FR-CNN. The fruit landmark based counting system has three steps: (1) it tracks fruits in 2D image plane (2) it estimate the camera poses and initialize fruit landmarks using SfM algorithm where the features are tracked fruits' centers instead of traditional geometrical features, (3) it tracks the landmarks by projecting them back to every image plane and match them with detections in every image (4) it counts the landmarks if it's observed in several frames and is before the tree centroids.

% To Remove: first track fruits in the image plane. The tracked fruits' centers are then used as feature correspondences across frames for the Structure from Motion (SfM) 3D reconstruction. The final data association is built by projecting the fruit landmarks reconstructed by the SfM algorithm back to every image and match them with the FR-CNN detections. Because we have both fruits' and trunks' 3D information, we use the tree centroid, which is assumed to have the same depth as the trunk, to avoid double counting of fruits. This step outputs a total count of fruits for the entire image sequence. Finally, we refine the final data association by locally optimizing the displacement of every fruit between every two frames, and obtain a final SfM 3D reconstruction, which contains camera pose estimates and a map of fruits.
% Our pipeline consists of the following parts: Firstly, we detect fruits in every image using a deep detection network, the Faster R-CNN (FR-CNN) and we segment trunks using a deep segmentation network. Secondly, we build an initial semantic data association, i.e. fruit feature matches across frames, by tracking fruits in the image plane. Thirdly, using the tracked fruits as feature correspondences, we build a Structure from Motion (SfM) 3D reconstruction. Fourthly, we build the final semantic data association by projecting the fruit landmarks reconstructed by the SfM algorithm back to every image and match them with the FR-CNN detections. Because we have both fruits' and trunks' 3D information, we use the tree centroid, which is assumed to have the same depth as the trunk, to avoid double counting of fruits. This step outputs a total count of fruits for the entire image sequence. Finally, we refine the final data association by locally optimizing the displacement of every fruit between every two frames, and obtain a final SfM 3D reconstruction, which contains camera pose estimates and a map of fruits.

